The Resource Problem of Using Linear Layer Leakage Attack in Federated Learning

Secure aggregation promises a heightened level of privacy in federated learning, maintaining that a server only has access to a decrypted aggregate update. Within this setting, linear layer leakage methods are the only data reconstruction attacks able to scale and achieve a high leakage rate regardless of the number of clients or batch size. This is done through increasing the size of an injected fully-connected (FC) layer. However, this results in a resource overhead which grows larger with an increasing number of clients. We show that this resource overhead is caused by an incorrect perspective in all prior work that treats an attack on an aggregate update in the same way as an individual update with a larger batch size. Instead, by attacking the update from the perspective that aggregation is combining multiple individual updates, this allows the application of sparsity to alleviate resource overhead. We show that the use of sparsity can decrease the model size overhead by over 327$\times$ and the computation time by 3.34$\times$ compared to SOTA while maintaining equivalent total leakage rate, 77% even with $1000$ clients in aggregation.

==> 5_additional_discussions.tex <==
% \subsection{FedAVG}
\iffalse
Over the course of a single FedAVG round, the parameters in the model will shift slightly. Since we use the same FC layer leakage methodology from Robbing the Fed, our application to FedAVG for the weights and biases of the layer follow the prior work. We also add a convolutional layer to the method. For this case, the parameters will change slightly when training each local mini-batch. These changes in the parameters are small and result in a minimal degradation of image quality~\cite{our2022mandrake}. We note that the size of the FC layer should be large enough for the size of the local client dataset in order to maintain a high leakage rate.
\fi

Unlike the gradients of the FC layers, the gradients of the convolutional layer are not necessary for the data reconstruction attack. A malicious server can then send a maliciously crafted model which would freeze the parameters of the convolutional layer to prevent changes from occurring over the local iterations of FedAVG. 

\iffalse
\subsection{Defenses}
Model architecture or parameter manipulation is much more difficult for clients in cross-device FL. As a result, clients must consider alternatives for privacy-preserving defenses. As discussed in this paper, secure aggregation (SA), or any other similar defense such as secure shuffling~\cite{kairouz2021advances}, is ineffective against linear layer leakage methods.

Differential privacy (DP) is also a commonly used method to preserve client data privacy in FL~\cite{dwork2014algorithmic, wei2020federated}. Particularly, if a client injects some noise into their model update, even a perfect reconstruction attack cannot recover the inputs without noise. This still holds true for linear layer leakage attacks. However, DP will hurt the model performance. Additionally, since the clients have no knowledge of when an attack will occur, they will be forced to apply DP for each participating training round. 
\fi
